X-ToM: Explaining with Theory-of-Mind for Gaining Justified Human Trust

We present a new explainable AI (XAI) framework aimed at increasing justified human trust and reliance in the AI machine through explanations. We pose explanation as an iterative communication process, i.e. dialog, between the machine and human user. More concretely, the machine generates sequence of explanations in a dialog which takes into account three important aspects at each dialog turn: (a) human's intention (or curiosity); (b) human's understanding of the machine; and (c) machine's understanding of the human user. To do this, we use Theory of Mind (ToM) which helps us in explicitly modeling human's intention, machine's mind as inferred by the human as well as human's mind as inferred by the machine. In other words, these explicit mental representations in ToM are incorporated to learn an optimal explanation policy that takes into account human's perception and beliefs. Furthermore, we also show that ToM facilitates in quantitatively measuring justified human trust in the machine by comparing all the three mental representations. We applied our framework to three visual recognition tasks, namely, image classification, action recognition, and human body pose estimation. We argue that our ToM based explanations are practical and more natural for both expert and non-expert users to understand the internal workings of complex machine learning models. To the best of our knowledge, this is the first work to derive explanations using ToM. Extensive human study experiments verify our hypotheses, showing that the proposed explanations significantly outperform the state-of-the-art XAI methods in terms of all the standard quantitative and qualitative XAI evaluation metrics including human trust, reliance, and explanation satisfaction.

==> sec4-relatedwork.tex <==
\section{Related Work}
Generating explanations or justifications of predictions or decisions made by an AI system has been widely explored in AI. Most prior work has focused on generating explanations using feature visualization and attribution.

\textbf{Feature visualization} techniques typically identify  qualitative interpretations of  features used for making predictions or decisions. 
Recently, there has been an increased interest in developing feature visualizations for deep learning models, especially for  Convolutional Neural Nets (CNNs) in computer vision applications, and  Recurrent Neural Nets (RNNs) in NLP applications.
For example, gradient ascent optimization is used in the image space to visualize the hidden feature layers of unsupervised deep architectures~\cite{erhan2009visualizing}. Also, convolutional layers are visualized by reconstructing the input of each layer from its output~\cite{zeiler2014visualizing}. Recent visual explanation models seek to jointly classify the image and explain why the predicted class label is appropriate for the image~\cite{hendricks2016generating}. Other related work includes a visualization-based explanation framework for Naive Bayes classifiers~\cite{greiner2003explaining}, an interpretable  character-level language models for analyzing the predictions in RNNs~\cite{karpathy2015visualizing}, and an interactive visualization for facilitating analysis of RNN hidden states \cite{strobelt2016visual}.

\textbf{Attribution} is a set of techniques that highlight pixels of the input image (saliency maps) that most caused the output classification. Gradient-based visualization methods~\cite{zhou2016learning,selvaraju2016grad} have been proposed to extract image regions responsible for the network output. The LIME method proposed by~\cite{ribeiro2016should} explains  predictions of any classifier by approximating it locally with an interpretable model.  Influence measures~\cite{datta2015influence} have been used to identify the importance of features in affecting the classification outcome for individual data points.

More recently, apart from feature visualization and attribution techniques, other important lines of research in explainable AI explore dimensionality reduction techniques~\cite{brinton17framework,maaten2008visualizing} and focus on building models which are intrinsically interpretable~\cite{zhang2017interpretable,stone2017teaching}. There are few recent works in the XAI literature that go beyond the pixel-level explanations. For example, the TCAV technique proposed by \cite{kim2018interpretability} aims to generate explanations based on high-level user defined concepts. Contrastive explanations are proposed by \cite{dhurandhar2018explanations} to identify minimal and sufficient features to justify the classification result. \cite{Goyal2019counterfactual} proposed counterfactual visual explanations that identify how the input could change such that the underlying vision system would make a different decision. More recently, few methods have been developed for building models which are intrinsically interpretable~\cite{zhang2017interpretable}. In addition, there are several works~\cite{miller2017explanation,hilton1990conversational,lombrozo2006structure} on the goodness measures of explanation which aim to understand the underlying characteristics of explanations. 

% We broadly categorize the trust based on the following two dimensions (similar to~\cite{}):\\
% \textbf{1. Sentiment}: Human's trust towards the machine is task-specific and multiple trusting relations can exist simultaneously. It is possible for humans to feel positive trust (PT) with respect to certain tasks and simultaneously feel negative trust (NT) (i.e. mis-trust, distrust, etc) on some other tasks. The definitions of PT and NT (equations (1) and (4)) and their derivation in continuous (equations (2) and (5)) and discrete (equations (3) and (6)) formulas are shown below. $\lambda$ is the hyperparameter and $p(I_t,T_t;\theta)$ denotes the joint prior over images $I$ and tasks $i$. In this work, we use uniform distribution over the number of sessions ($1/N$) as the prior. 
% %\begin{equation}
% %\displaystyle\sum_{z=\alpha,\beta,\gamma}\dfrac{\|pg_{zt}^{AinU} \cap pg_{zt}^{U}\|}{\|pg_{zt}^{A} \cup pg_{zt}^{AinU} \cup pg_{zt}^{U}\|}
% \begin{align}
% \text{PT} &= \displaystyle\int_{t}^{}\Delta \text{PT}(t)\: p(I_t,T_t;\theta) \: dt\\ 
% \Delta \text{PT}(t) &= e^{-\lambda/\:\|pg^{MinU}_{t,+}\|}\\
% \text{PT} &= \displaystyle\sum_{i}\Delta \text{PT}(i)\: p(I_i,T_i;\theta)\\
% \Delta \text{PT}(i)  &= \displaystyle\dfrac{\|pg^{MinU}_{i,+}\|}{\|pg_{i}^{M} \cup pg_{i}^{MinU}\|}\\
% \\
% \text{JPT} &= \displaystyle\int_{t}^{}\Delta \text{JPT}(t)\: p(I_t,T_t;\theta) \: dt\\ 
% \Delta \text{JPT}(t) &= e^{-\lambda\:\text{KL}\left(pg^{MinU}_{t,+} || pg^{M}_{t,+}\right)}\\
% \text{JPT} &= \displaystyle\sum_{i}\Delta \text{JPT}(i)\: p(I_i,T_i;\theta)\\
% \Delta \text{JPT}(i)  &= \displaystyle\dfrac{\|pg^{MinU}_{i,+} \cap pg^{M}_{i,+}\|}{\|pg_{i}^{M} \cup pg_{i}^{MinU}\|}\\
% \\
% \text{NT} &= \displaystyle\int_{t}^{}\Delta \text{NT}(t)\: p(I_t,T_t;\theta) \: dt\\ 
% \Delta \text{NT}(t) &= e^{-\lambda/\:\|pg^{MinU}_{t,-}\|}\\
% \text{NT} &= \displaystyle\sum_{i}\Delta \text{NT}(i)\: p(I_i,T_i;\theta)\\
% \Delta \text{NT}(i)  &= \displaystyle\dfrac{\|pg^{MinU}_{i,-}\|}{\|pg_{i}^{M} \cup pg_{i}^{MinU}\|}\\
% \\
% \text{JNT} &= \displaystyle\int_{t}^{}\Delta \text{JNT}(t)\: p(I_t,T_t;\theta) \: dt\\ 
% \Delta \text{JNT}(t) &= e^{-\lambda\:\text{KL}\left(pg^{MinU}_{t,-} || pg^{M}_{t,-}\right)}\\
% \text{JNT} &= \displaystyle\sum_{i}\Delta \text{JNT}(i)\: p(I_i,T_i;\theta)\\
% \Delta \text{JNT}(i)  &= \displaystyle\dfrac{\|pg^{MinU}_{i,-} \cap pg^{M}_{i,-}\|}{\|pg_{i}^{M} \cup pg_{i}^{MinU}\|}\\
% \end{align}
% \textbf{Reliance}: It is possible that humans might over-estimate or under-estimate the capability of the system. Reliance (RC) captures the extent to which human can predict the machine's understanding without over-estimating or under-estimating it. 
% %Reliance measures the positive and negative trust
% %The positive and negative trust of humans towards a machine can be a mixture of justified trust (JT) and unjustified trust (UT). Reliance is Justified Positive Trust measures the aspect of reliance on the system (i.e. positive trust + negative trust). In our experiments (see section 5.3), we found that unjustified trust arises mainly due to either over-estimating or under-estimating the competence of the system.  We use the equations (3) and (4) to estimate JT and UT.
% %\begin{equation}
% %\begin{aligned}
% %P\left( \left(|pg^{MinU} \cap pg^M| \geq \epsilon\right) \;\middle|\; \left(|pg^M \cap pg^U| \leq \epsilon\right)\right) \geq \delta
% %\end{aligned}
% %\end{equation}
% %\begin{equation}
% %\begin{aligned}
% %P\left( \left(|pg^{MinU} \cap pg^M| \leq \epsilon\right) \;\middle|\; \left(|pg^M \cap pg^U| \geq \epsilon\right)\right) \geq \delta
% %\end{aligned}
% %\end{equation}
% %\begin{equation}

% Reliance (RC) \approx \text{Justified PT} + \text{Justified NT}

% \begin{align}
% \text{RC} &= \displaystyle\int_{t}^{}\Delta \text{RC}(t)\: p(I_t,T_t;\theta) \: dt\\ 
% \Delta \text{RC}(t) &= e^{-\lambda\:\text{KL}\left(pg^{MinU}_t || pg^{M}_t\right)}\\
% \text{RC} &= \displaystyle\sum_{i}\Delta \text{RC}(i)\: p(I_i,T_i;\theta)\\
% \Delta\text{RC}(t) &= \displaystyle\dfrac{\|pg^{MinU}_{i} \cap pg^{M}_{i}\|}{\|pg_{i}^{M} \cup pg_{i}^{MinU}\|}
% \end{align}


%\section{Sari Related work}
%Another approach to explainable AI is to view explanation generation as primarily a language generation problem. Models from this brand often utilize deep learning not only to make a decision but also a matching explanation \cite{DBLP:journals/corr/HendricksARDSD16,DBLP:journals/corr/abs-1802-08129,DBLP:journals/corr/HarrisonER17}. While this type of models show promising results, when considering the models reliance on a black box to generate the explanation itself - and not to mention the fact that the the explanation does not necessarily describe the inner working of the decision making models - it becomes clear that these models are addressing a completely different problem. In fact, the term \textit{Rationalization} have been used to differentiate this approach from the conventional explanation body of work  \cite{journals/corr/HarrisonER17}.

==> subsec2.2-mind-representation.tex <==
%As illustrated Figure~\ref{fig:framework}, 
\subsection{Representation of Minds in X-ToM} \label{mind-representation}
The three minds $pg^{M}$, $pg^{MinU}$, and $pg^{UinM}$ are sub-graphs of an And-Or Graph (AOG) defining all objects, parts, and their relationships and attributes of the visual domain considered. Our motivation to use AOGs for modeling the three mental states of the Theory of Mind stems from the following advantages. First, an AOG is a context-sensitive stochastic grammar~\cite{zhu2007stochastic} that can explicitly capture rich contextual and hierarchical relationships (spatial, temporal and causal). Second, AOG based representation and inference is a domain generic approach and the literature has abundantly demonstrated that AOG based systems, especially recent methods that combine deep learning and AOGs, are the top performers for a wide range of tasks in domains such as computer vision, natural language processing, and human-robot collaboration~\cite{zhang2017interpretable,liu2016jointly,wu2011numerical,tu2014joint,park2016attribute}. Third, since the result of visual recognition (i.e., a parse graph) is a sub-graph of the AOG, image interpretations can be readily explained using the top-down, bottom-up, or contextual types of visual reasoning enabled by the AOG. Finally, and of great importance for XAI systems, the rich contextual and hierarchical nature of AOGs allows for formalizing and quantitatively evaluating human trust in the visual performer along both depth and breadth.

\noindent
\textbf{As AOG is interpretable, why not show $Pg^M$ directly to the user as an explanation?} 
It will be daunting to show the entire AOG since our AOG encodes hundreds of objects, parts, activities, attributes and other concepts as nodes. In addition, AOG has numerous edges. It might be possible to visualize a part of AOG, but it is not clear how to optimize which AOG subgraph would not overwhelm the user and maximize utility. The advantage of using our dialog based explanations is that, at each dialog turn, explainer can tailor the explanations based on the user’s current perception and understanding (Miller et al., 2017).

